An Introduction to the Deviatoric Decomposition in Three-Dimensions Based on a Recursive Formula

Higher-order tensors appear in various areas of mechanics as well as physics, medicine or earth sciences. As these tensors are highly complex, most are not well understood. Thus, the analysis and the visualization process form a highly challenging task. In order to solve this problem a suitable tensor decomposition for arbitrary tensors is desirable. Since many real-world examples are described in the three-dimensional space, this paper will also focus on this space. Tensors of order zero and one are well understood and for second order tensors the well-known spectral decomposition exists. However, there is no standard decomposition for tensors of order higher than two. This work will focus on summarizing facts about the deviatoric decomposition and on its calculation in a recursive way. It decomposes a tensor of arbitrary order into a sum of orthogonal, irreducible parts. Thus, into parts that are orthogonal and invariant under rotation. These irreducible parts are based on so-called deviators. The calculations and results of the deviatoric decomposition are not broadly understood in the engineering community. To change this situation, information about this decomposition from a range of literature sources was gathered and will be summarized and explained in this work to make further analysis possible. Different applications and examples for often used physical tensors will also be given. The goal of this work is to give other researchers the chance to also use this knowledge.

==> Content/DevDecThirdOrder4.tex <==
\begin{equation}\label{eq:RecformulaThird}
	\begin{split}
		T_{ijk} =& I_{jk}^{(2,0)J} d_i^1 + I_{jk}^{(2,1)1} \left[ d^1 \delta_{mi} + \varepsilon_{mis} d_s^1 + D_{mi} \right]\\
		& + I_{jk}^{(2,2)1}\left[ L_{in_1 n_2 m} D_m + \varepsilon_{it\hat{n}_1} D_{\hat{n}_2 t + D_{in_1 n_2}} \right]\\
		=& \delta_{jk} d_i^1 + \varepsilon_{jks}\delta_{si}d^1 + \varepsilon_{jkm}\varepsilon_{mis}d_s^1 + \varepsilon_{jks}D_{si} + L_{ijks} D_s + \varepsilon_{it\hat{j}}D_{\hat{k}t} + D_{ijk}\\
		=& \varepsilon_{jki}d + \delta_{jk} d_i^1 + \varepsilon_{jkm}\varepsilon_{mis}d_s^2 + L_{ijks}d_s^3 + \varepsilon_{jks}D_{si}^1 + \varepsilon_{is\hat{j}}D_{\hat{k}s}^2 + D_{ijk} \\
		=& \varepsilon_{ijk}d + \delta_{jk}d_i^1 + \varepsilon_{jkm}\varepsilon_{mis}d_s^2 + L_{ijks}d_s^3 + \varepsilon_{jks}D_{si}^1 + \varepsilon_{is\hat{j}}D_{\hat{k}s} + D_{ijk}.
	\end{split}
\end{equation}
Thus, it is
\begin{equation}
\begin{split}
	T_{ijk} =& \varepsilon_{ijk}d + \delta_{jk}d_i^1 \\
	&+ \varepsilon_{jk1}\varepsilon_{1i2}d_2^2 + \varepsilon_{jk1}\varepsilon_{1i3}d_3^2 \\
	& + \varepsilon_{jk2}\varepsilon_{2i1}d_1^2 + \varepsilon_{jk2}\varepsilon_{2i3}d_3^3 \\
	&+ \varepsilon_{jk3}\varepsilon_{3i1}d_1^2 + \varepsilon_{jk3}\varepsilon_{3i2}d_2^2 \\
	&+ \left( \frac{3}{2} \left( \delta_{ij}\delta_{k1} + \delta_{ik} \delta_{j1}\right) - \delta_{i1}\delta_{jk}\right) d_1^3 \\
	&+ \left( \frac{3}{2} \left( \delta_{ij}\delta_{k2} + \delta_{ik}\delta_{j2}\right) - \delta_{i2}\delta_{jk}\right) d_2^3 \\
	&+ \left( \frac{3}{2} \left( \delta_{ij}\delta_{k3} + \delta_{ij}\delta_{j3}\right) - \delta_{i3}\delta_{jk}\right) d_3^3\\
	&+ \varepsilon_{jk1}D_{1i}^1 + \varepsilon_{jk2}D_{2i}^1 + \varepsilon_{jk3}D_{3i}^1\\
	&+ \frac{1}{2} \left( \varepsilon_{i1j}D_{k1}^2 + \varepsilon_{i1k}D_{j1}^2 + \varepsilon_{i2j}D_{k2}^2 + \varepsilon_{i2k}D_{j2}^2 + \varepsilon_{i3j}D_{k3} + \varepsilon_{i3k}D_{j3} \right) \\
	&+ D_{ijk}.
\end{split}
\end{equation}
This result can be summarized to
\begin{equation}
\begin{split}
	&T_{iii} = d_i^1 + 2d_i^3 + D_{iii}\\
	&T_{ijj} = d_i^1 - d_i^3 + \varepsilon_{ilj}D_{jl}^2 + D_{ijj}\\
	&T_{iij} = \varepsilon_{ijl}\varepsilon_{lij}d_j^2 + \frac{3}{2} d_j^3 + \varepsilon_{ijl}D_{li}^1 + \frac{1}{2}\varepsilon_{ilj}D_{il}^2 + D_{iij} \\
	&T_{iji} = \varepsilon_{jil}\varepsilon_{lim}d_m^2 + \frac{3}{2} d_j^3 + \varepsilon_{jil}D_{li}^1 + \frac{1}{2}\varepsilon_{ilj}D_{il}^2 + D_{iji}\\
	&T_{ijk} = \varepsilon_{ijk} d + \varepsilon_{jkn}D_{ni}^1 + \frac{1}{2}\left( \varepsilon_{imj}D_{km}^2 + \varepsilon_{ink}D_{jn}^2 \right) + D_{ijk},
\end{split}
\end{equation}
where $j\neq l\neq i$, $l\neq m\neq i, \, i\neq n \neq k$ 
  and $i\neq j\neq k \neq i$.
These coefficients can be used to generate an equation system 
  to calculate equations for the deviators.
Therefore, the \gls{doubleContraction} with the
  \gls{kroneckerDelta} $\delta_{ij}$ or the
  \gls{permutationTensor} 
  $\varepsilon_{ijk}$ with the general third-order tensor 
  $\third{T}$ must be calculated:
\begin{equation}
\begin{split}
T_{ijj}\delta_{ij} &= T_{111} + T_{122} + T_{133} \\
&= d_1^1 + 2d_1^3 + D_{111} + d_1^1 - d_1^3 - D_{23}^2 + D_{122} + d_1^1 - d_1^3 + D_{23}^2 + D_{133}\\
&= 3d_1^1\\
T_{1ij}\varepsilon_{ij1} &= \varepsilon_{231}T_{123} + \varepsilon_{321}T_{132} = T_{123} - T_{132}\\
&= d + D_{11}^1 -\frac{1}{2}D_{33}^2 + \frac{1}{2} D_{22}^2 + D_{123} \\
 & \qquad - \left( -d -D_{11^1}-\frac{1}{2} D_{33}^2 + \frac{1}{2}D_{22}^2 + D_{123} \right) \\
&= 2d + 2D_{11}^1.
\end{split}
\end{equation}
There are 34 other contractions of this kind.
The contractions with the Kronecker delta 
\begin{equation}
\begin{split}
T_{2ij}\delta_{ij} &= 3d_2^1 \\
T_{3ij}\delta_{ij} &= 3d_3^1\\
T_{ij1}\delta_{ij} &= d_1^1 + 2d_1^2 + 5d_1^3 \\
T_{ij2}\delta_{ij} &= d_2^1 + 2d_2^2 + 5d_2^3 \\
T_{ij3}\delta_{ij} &= d_3^1 + 2d_3^2 + 5d_3^3 \\
T_{i1j}\delta_{ij} &= d_1^1 - 2d_1^2 + 5d_1^3 \\
T_{i2j}\delta_{ij} &= d_2^1 - 2d_2^2 + 5d_2^3 \\
T_{i3j}\delta_{ij} &= d_3^1 - 2d_3^2 + 5d_3^3 
\end{split}
\end{equation}
can be used to calculate the three first-order deviators $\first{d}^1, \, \first{d}^2$ and $\first{d}^3$.
These results and the contractions with the permutation tensor
\begin{equation}
\begin{split}
T_{1ij}\varepsilon_{ij1} &= 2d + 2D_{11}^1, \quad T_{2ij}\varepsilon_{ij2} = 2d + 2D_{22}^1, \quad T_{3ij}\varepsilon_{ij3} = 2d + 2D_{33}^1\\
T_{1ij}\varepsilon_{ij2} &= -2d_3^2 + 2D_{12}^1, \quad T_{1ij}\varepsilon_{ij3} = 2d_2^2 + 2D_{13}^1 , \quad
T_{2ij}\varepsilon_{ij1} = 3d_3^2 + 2D_{12}^1\\
T_{2ij}\varepsilon_{ij3} &= -2d_1^2 + 2D_{23}^1, \quad T_{3ij}\varepsilon_{ij1} = -2d_2^2 + 2D_{12}^1, \quad T_{3ij}\varepsilon_{ij2} = 2d_1^2 + 2D_{23}^1\\
T_{ij1}\varepsilon_{ij1} &= 2d + D_{22}^1 + D_{33}^1- D_{11}^2 + \frac{1}{2}D_{22}^2 + \frac{1}{2}D_{33}^2\\
T_{ij2}\varepsilon_{ij2} &= 2d+ D_{11}^1 + D_{33}^1-D_{22}^2 + \frac{1}{2}D_{11}^2 + \frac{1}{2}D_{22}^2\\
T_{ij1}\varepsilon_{ij2} &= d_3^1 + d_3^2 -\frac{5}{2}d_3^3 - D_{12}^1 -\frac{3}{2}D_{12}^2\\
T_{ij1}\varepsilon_{ij3} &= -d_2^1 - d_2^2 + \frac{5}{2}d_2^3 - D_{13}^1 - \frac{3}{2}D_{13}^2\\
T_{ij2}\varepsilon_{ij1} &= -d_3^1 - d_3^2 + \frac{5}{2}d_3^3 - D_{12}^1 - \frac{3}{2}D_{12}^2\\
T_{ij2}\varepsilon_{ij3} &= d_1^1+ d_1^2 - \frac{5}{2}d_1^3 - D_{23}^1 - \frac{3}{2}D_{23}^2 \\
T_{ij3}\varepsilon_{ij1} &= d_2^1 + d_2^2 - \frac{5}{2}d_2^3 - D_{13}^1 - \frac{3}{2}D_{13}^2\\
T_{ij3}\varepsilon_{ij2} &= -d_1^1 - d_1^2 -\frac{5}{2}d_1^3 - D_{23}^1 - \frac{3}{2}D_{23}^2\\
T_{i1j}\varepsilon_{ij1} &=-2d - D_{22}^1 - D_{33}^1 - D_{11}^2 + \frac{1}{2}D_{22}^2 + \frac{1}{2}D_{33}^2\\
T_{i2j}\varepsilon_{ij2} &= - 2d- D_{11}^1 - D_{33}^1 - D_{22}^2 + \frac{1}{2}D_{11}^2 + \frac{1}{2}D_{33}^2\\
T_{i3j}\varepsilon_{ij3} &= -2d-D_{11}^1- D_{22}^1 -D_{33}^2 + \frac{1}{2} D_{22}^2+ \frac{1}{2}D_{11}^2\\
T_{i1j}\varepsilon_{ij2} &= d_3^1 - d_3^2 - \frac{5}{2}d_3^3 + D_{12}^1 - \frac{3}{2}D_{12}^2\\
T_{i1j}\varepsilon_{ij3} &= - d_2^1 + d_2^2 + \frac{5}{2}d_2^3 + D_{13}^1 - \frac{3}{2}D_{13}^2\\
T_{i2j}\varepsilon_{ij1} &= -d_3^1 + d_3^2 + \frac{5}{2}d_3^3 + D_{12}^1 - \frac{3}{2}D_{12}^2\\
T_{i2j}\varepsilon_{ij3} &= d_1^1 - d_1^2 - \frac{5}{2}d_1^3 + D_{23}^1 - \frac{3}{2}D_{23}^2\\
T_{i3j}\varepsilon_{ij1} &= d_2^1 - d_2^2 - \frac{5}{2}d_2^3 + D_{13}^1 - \frac{3}{2}D_{13}^2\\
T_{i3j}\varepsilon_{ij2} &= -d_1^1 + d_1^2 + \frac{5}{2}d_1^3 + D_{23}^1 - \frac{3}{2}D_{23}^2
\end{split}
\end{equation}
can be used to calculate the zeroth-order deviator $d$ and the two
  second-order deviators $\second{D}^1$ and $\second{D}^2$.
The zeroth-order deviator $d$ is given by
\begin{equation}
	d= \frac{1}{6} \left( T_{123} - T_{132}- T_{213}+T_{231}+ T_{312}- T_{321}\right),
\end{equation}
the three first-order deviators $\first{d}^1, \, \first{d}^2$ 
  and $\first{d}^3$ by 
\begin{equation}
\begin{split}
d^1 = \frac{1}{3} \begin{pmatrix}
T_{111} + T_{122} + T_{133}\\
T_{211} + T_{222} + T_{233}\\
T_{311} + T_{322} + T_{333}
\end{pmatrix}, \qquad d^2 =\frac{1}{4} \begin{pmatrix}
T_{221}-T_{212}+ T_{331}-T_{313}\\
T_{112} - T_{121}+ T_{332} - T_{323}\\
T_{113} - T_{131}+ T_{223} - T_{232}
\end{pmatrix}\\
d^3 =\frac{1}{30} \begin{pmatrix}
4T_{111} - 2T_{122}-2T_{133}+ 3T_{221}+ 3T_{331}+3T_{212}+3T_{313}\\
4T_{222} - 2T_{211}-2T_{233}+3T_{112}+3T_{332} +3T_{121}+3T_{323}\\
4T_{333}-2T_{311}-2T_{322}+3T_{113}+3T_{223}+3T_{131}+3T_{232}
\end{pmatrix}
\end{split}
\end{equation}
and the two second-order deviators $\second{D}^1$ and $\second{D}^2$ by
\begin{equation}
\begin{split}
&D_{11}^1 = \frac{1}{6} \left( 2T_{123}-2T_{132}+T_{213}-T_{231}-T_{312}+T_{321}\right) \\
&D_{22}^1 = \frac{1}{6} \left( -T_{123}+T_{132}-2T_{213}+2T_{231}-T_{312}+T_{321}\right) \\
&D_{33}^1 = \frac{1}{6} \left( -T_{123}+T_{132}+T_{213}-T_{231}+2T_{312}-2T_{321}\right)\\
&D_{12}^1 = \frac{1}{4}\left( -T_{113}+T_{131}+T_{223}-T_{232}\right) \\
&D_{13}^1 = \frac{1}{4}\left( T_{112}-T_{121}+T_{323}-T_{332}\right)\\
&D_{23}^1 = \frac{1}{4}\left( T_{212}-T_{221}-T_{313}+T_{331}\right),\\
\\
&D_{11}^2 = \frac{1}{3}\left( - T_{213}-T_{231}+T_{312}+T_{321}\right)\\
&D_{22}^2 = \frac{1}{3}\left( T_{123} + T_{132} - T_{312} -T_{321}\right) \\
&D_{33}^2 = \frac{1}{3}\left( -T_{123} - T_{132}+ T_{213} + T_{231}\right)\\
&D_{12}^2 = \frac{1}{6} \left( T_{113} + T_{131} - T_{223} - T_{232} -2T_{311}+ 2T_{322} \right)\\
&D_{13}^2 = \frac{1}{6} \left( -T_{112} - T_{121} + 2T_{211} - 2T_{233} + T_{323} + T_{332} \right) \\
&D_{23}^2 = \frac{1}{6} \left( -2T_{122} + 2T_{133} + T_{212} + T_{221} -T_{313} -T_{331}\right).
\end{split}
\end{equation}
These deviators and \autoref{eq:RecformulaThird} can be used to
  calculate the third-order deviator
\begin{equation}
\begin{split}
&D_{111} = \frac{2}{5}T_{111}-\frac{1}{5}T_{122}-\frac{1}{5}T_{133}-\frac{1}{5}T_{221}-\frac{1}{5}T_{331}-\frac{1}{5}T_{212}-\frac{1}{5}T_{313}\\
&D_{222} = \frac{2}{5}T_{222}-\frac{1}{5}T_{211}-\frac{1}{5}T_{233}-\frac{1}{5}T_{112}-\frac{1}{5}T_{332}-\frac{1}{5}T_{121}-\frac{1}{5}T_{323}\\
&D_{333} = \frac{2}{5}T_{333}-\frac{1}{5}T_{322}-\frac{1}{5}T_{311}-\frac{1}{5}T_{113}-\frac{1}{5}T_{223}-\frac{1}{5}T_{131}-\frac{1}{5}T_{232}\\
&D_{122} = \frac{4}{15}T_{122}- \frac{1}{5}T_{111}-\frac{1}{15}T_{133}+\frac{4}{15}T_{221}-\frac{1}{15}T_{331}-\frac{1}{15}T_{313}+ \frac{4}{15}T_{212}\\
&D_{133} = \frac{4}{15}T_{133} - \frac{1}{5}T_{111} - \frac{1}{15}T_{221} + \frac{4}{15}T_{331} + \frac{4}{15}T_{313}-\frac{1}{15}T_{212}-\frac{1}{15}T_{122}\\
&D_{211} = \frac{4}{15}T_{211}-\frac{1}{5}T_{222}- \frac{1}{15}T_{233} + \frac{4}{15}T_{112} + \frac{4}{15} T_{121}- \frac{1}{15}T_{332} - \frac{1}{15}T_{323}\\
&D_{233} = \frac{4}{15}T_{233}- \frac{1}{15}T_{211}-\frac{1}{5}T_{222} - \frac{1}{15}T_{112} -\frac{1}{15}T_{121}+ \frac{4}{15}T_{332}+ \frac{4}{15}T_{323}\\
&D_{311} = \frac{4}{15} T_{311} - \frac{1}{15}T_{322} -\frac{1}{5}T_{333}+ \frac{4}{15}T_{113} + \frac{4}{15}T_{131}-\frac{1}{15}T_{223}-\frac{1}{15}T_{232}\\
&D_{322} = \frac{4}{15}T_{322}- \frac{1}{15}T_{311}-\frac{1}{15}T_{333}-\frac{1}{15}T_{113} - \frac{1}{15}T_{131}+ \frac{4}{15}T_{223}+ \frac{4}{15}T_{232}\\
&D_{123} = \frac{1}{6}T_{123} + \frac{1}{6}T_{132}+ \frac{1}{6}T_{213}+ \frac{1}{6}T_{231} + \frac{1}{6}T_{312} + \frac{1}{6}T_{321}.
\end{split}
\end{equation}
\\
\textbf{Third-Order Coupling Tensor.}
For the third-order coupling tensor $\third{H}$ with
  $H_{ijk}=H_{jik}$ the deviators of the previous 
  paragraph can be simplified to
\begin{equation}
\begin{split}
	&\first{d}^2 = \frac{1}{4} \begin{pmatrix}
	H_{221} - H_{122} + H_{331} - H_{133}\\
	H_{112} - H_{121} + H_{332} - H_{233} \\
	H_{133} - H_{131} + H_{223} - H_{232}
	\end{pmatrix}\\
	&\first{d}^3 = \frac{1}{30} \begin{pmatrix}
	4H_{111} + H_{122} + H_{133} + 3H_{221} +3H_{331}\\
	4H_{222} + H_{121} + H_{233} + 3H_{112} +3H_{332}\\
	4H_{333} + H_{131} + H_{232} + 3H_{113} +3H_{223}
	\end{pmatrix},
\end{split}
\end{equation}
and
\begin{equation}
\begin{split}
&D_{11}^1 = \frac{1}{2}\left( H_{123} - H_{132}\right)\\
&D_{22}^1 = \frac{1}{2}\left( H_{231} - H_{123}\right)\\
&D_{33}^1 = \frac{1}{2}\left( H_{132} - H_{231}\right)\\
&D_{12}^1 = \frac{1}{4}\left(-H_{113}+H_{131}+H_{223}-H_{232}\right)\\
&D_{13}^1 = \frac{1}{4}\left( H_{112}-H_{121}+H_{233}-H_{332}\right)\\
&D_{23}^1 = \frac{1}{4}\left( H_{122}-H_{221}-H_{133}+H_{331}\right)
\end{split}
\end{equation}
and 
\begin{equation}
\begin{split}
&D_{111} = \frac{2}{5} H_{111} - \frac{2}{5}H_{122} - \frac{2}{5}H_{133} - \frac{1}{5}H_{221} -\frac{1}{5}H_{331}\\
&D_{222} = \frac{2}{5}H_{222}-\frac{2}{5}H_{211}-\frac{2}{5}H_{233}-\frac{1}{5}H_{112} - \frac{1}{5} H_{332}\\
&D_{333} = \frac{2}{5}H_{333}-\frac{2}{5}H_{322}-\frac{2}{5}H_{311}-\frac{1}{5}H_{113}-\frac{1}{5}H_{223}\\
&D_{122} = \frac{8}{15}H_{122}-\frac{1}{5}H_{111}-\frac{2}{15}H_{133}+\frac{4}{15}H_{221}-\frac{1}{15}H_{331}\\
&D_{133} = \frac{8}{15}H_{133}-\frac{1}{5}H_{111}-\frac{1}{15}H_{221}+\frac{4}{15}H_{331}-\frac{2}{15}H_{212}\\
&D_{211} = \frac{8}{15}H_{211}-\frac{1}{5}H_{222}-\frac{2}{15}H_{233}+ \frac{4}{15}H_{112}-\frac{1}{15}H_{332}\\
&D_{233} = \frac{8}{15}H_{233}-\frac{2}{15}H_{211}-\frac{1}{5}H_{222} -\frac{1}{15}H_{112}+ \frac{4}{15}H_{332}\\
&D_{311} = \frac{8}{15}H_{311}-\frac{2}{15}H_{322}-\frac{1}{5}H_{333}+\frac{4}{15}H_{113}-\frac{1}{15}H_{223}\\
&D_{322} = \frac{8}{15}H_{322}-\frac{2}{15}H_{311}-\frac{1}{5}H_{333}-\frac{1}{15}H_{113} + \frac{4}{15}H_{223}\\
&D_{123}= \frac{1}{3}H_{123} + \frac{1}{3}H_{132} + \frac{1}{3}H_{231}.
\end{split}
\end{equation}
%
For the deviators $d$, $\first{d}^1$ and $\second{D}^2$
  it is
\begin{equation}
\begin{split}
d = 0, \quad \first{d}^1 = \frac{5}{2} \first{d}^3 - \first{d}_2, \quad D_{ij}^2 = -\frac{2}{3}D_{ij}^1.
\end{split}
\end{equation}
%
Thus, the coupling tensor can be represented by
  four deviators: two of order one, one of order two
  and one of order three.\\
\\
